Overlap Local-SGD: An Algorithmic Approach to Hide Communication Delays in Distributed SGD

Distributed stochastic gradient descent (SGD) is essential for scaling the machine learning algorithms to a large number of computing nodes. However, the infrastructures variability such as high communication delay or random node slowdown greatly impedes the performance of distributed SGD algorithm, especially in a wireless system or sensor networks. In this paper, we propose an algorithmic approach named Overlap-Local-SGD (and its momentum variant) to overlap the communication and computation so as to speedup the distributed training procedure. The approach can help to mitigate the straggler effects as well. We achieve this by adding an anchor model on each node. After multiple local updates, locally trained models will be pulled back towards the synchronized anchor model rather than communicating with others. Experimental results of training a deep neural network on CIFAR-10 dataset demonstrate the effectiveness of Overlap-Local-SGD. We also provide a convergence guarantee for the proposed algorithm under non-convex objective functions.

==> 3_result.tex <==
\section{Related Works}\label{sec:related}
The idea of pulling back locally trained models towards an anchor model is inspired by elastic averaging SGD (EASGD) \cite{Zhang2015elasticsgd}, which allows some slack between local models by adding a proximal term to the objective function. The convergence guarantee of EASGD under non-convex objectives has not been established until our recent work \cite{wang2018cooperative}. However, in EASGD, the anchor and local models are updated in a symmetric manner (\ie, mixing matrix $\bW_k$ in \eqref{eqn:update} should be symmetric and doubly-stochastic). EASGD naturally allows overlap of communication and computation, but the original paper \cite{Zhang2015elasticsgd} did not observe and utilize this advantage to reduce communication delays. %\GJ{Avoid saying 'Did not realize'. Can instead say -- EASGD naturally allows overlap of communication and computation, but the original paper \cite{Zhang2015elasticsgd} did not observe and utilize this advantage to reduce communication delays}

There also exist other techniques that can decouple communication and computation in Local SGD. In \cite{Shen2019FasterDD}, the authors propose to apply the local updates to an averaged model which is $\cp$-iterations before. Their proposed algorithm CoCoD-SGD can achieve the same runtime benefits as {\alg}. Nonetheless, later in \Cref{sec:exps}, we will show that {\alg} consistently reaches comparable or even higher test accuracy than CoCoD-SGD given the same $\cp$. {In a concurrent work \cite{wang2019osp}, the authors develop a similar method to CoCoD-SGD.}

\section{Experimental Results}\label{sec:exps}

\textbf{Experimental setting.} The experimental analysis is performed on CIFAR-10 image classification task \cite{krizhevsky2009cifar}. We train a ResNet-18 \cite{he2016deep} for $300$ epochs following the exactly same training schedule as \cite{vogels2019powersgd}. That is, the mini-batch size on each node is $128$ and the base learning rate is $0.1$, decayed by $10$ after epoch $150$ and $250$. The first 5 epochs use the learning rate warmup schedule as described in \cite{goyal2017accurate}. There are $16$ computing nodes in total connected via $40$ Gbps Ethernet, each of which is equipped with one NVIDIA Titan X GPU. The training data is evenly partitioned across all nodes and \emph{not shuffled} during training. The algorithms are implemented in PyTorch \cite{paszkepytorch} and NCCL communication backend.

In {\alg}, the momentum factor of the anchor model is set to $\beta=0.7$, following the convention in \cite{wang2019slowmo}. For different number of local updates $\cp$, we tune the value of pullback parameter $\glr$. It turns out that in the considered training task, for $\cp\geq2$, $\glr=0.6$ consistently yields the best test accuracy at convergence. In intuition, a larger value of $\glr$ may enable a larger learning rate. We believe that if one further tune the base learning rate and the momentum factor, the performance of {\alg} will be further improved. For example, in our setting, when $\cp=1$, then $\glr=0.5$ and base learning rate $0.15$ gives the highest accuracy.

\begin{figure*}[!hbtp]
    \centering
    \begin{subfigure}{.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{comparison_iid.pdf}
    \caption{Error-runtime trade-off.}
    \end{subfigure}%
    ~
    \begin{subfigure}{.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{error_time_iid.pdf}
    \caption{Validation curves.}
    \end{subfigure}%
    ~
    \begin{subfigure}{.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{loss_epoch_iid.pdf}
    \caption{Training curves.}
    \end{subfigure}
    \caption{Comparison of communication-efficient SGD methods in \textbf{IID} data partition setting. In (a), the number of local updates of Local SGD method is taken from $\{1,2,4,8,24\}$. In (b) and (c), we fix $\cp=2$. (Best viewed in color)}
    \label{fig:IID}
\end{figure*}

\begin{figure*}[t]
    \centering
    \begin{subfigure}{.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{comparison_niid.pdf}
    \caption{Error-runtime trade-off.}
    \end{subfigure}%
    ~
    \begin{subfigure}{.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{error_time_niid.pdf}
    \caption{Validation curves.}
    \end{subfigure}%
    ~
    \begin{subfigure}{.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{loss_epoch_niid.pdf}
    \caption{Training curves.}
    \end{subfigure}
    \caption{Comparison of communication-efficient SGD methods in \textbf{non-IID} data partition setting. In (a), the number of local updates of Local SGD method is taken from $\{1,2,4,8,24\}$. In (b) and (c), we fix $\cp=2$. {\alg} is much more stable than other methods.}
    \label{fig:NIID}
    \vspace{-8pt}
\end{figure*}

\textbf{Negligible Communication Cost.}
We first examine the effectiveness of the overlap technique. As shown in \Cref{fig:IID}(a), {\alg} significantly outperforms all other methods. Given a target final accuracy, {\alg} incurs nearly negligible additional latency compared to fully synchronous SGD ($0.1$s versus $1.5$s per epoch). When $\cp=2$, {\alg} reduces the communication-to-computation ratio from $34.6\%$ to $1.5\%$, while maintaining roughly the same loss-versus-iterations convergence as fully synchronous SGD (see \Cref{fig:IID}(c)). The superiority of {\alg} will be further magnified when using a slow inter-connection (\eg, $10$ Gbps) or a larger neural network (\eg, transformer \cite{ott2018scaling}).

Compressing or quantizing the exchanged gradients among worker nodes is another communication-efficient training method, which is extensively studied in recent literature. Here, we choose PowerSGD \cite{vogels2019powersgd}, which is the state-of-the-art gradient compression algorithm, as another baseline to compare with. In \Cref{fig:IID}, the rank of PowerSGD ranges from $\{1,2,4,8\}$ (lower means higher compression ratio). When the rank is 1 (the lowest), PowerSGD can compress the transferred gradient by $243\times$. However, even in this extreme case, the additional synchronization latency of PowerSGD is still much higher than Local SGD methods. The reason is that the nodes cost some time to establish the handshakes. Compression techniques cannot reduce this part of communication overhead, and also introduce non-negligible encoding and decoding latency.

\textbf{Higher Accuracy than Other Local SGD Variants.} As discussed in \Cref{sec:related}, EASGD (and its momentum version EAMSGD \cite{Zhang2015elasticsgd}) also involve(s) a similar `pullback' mechanism as {\alg}. And CoCoD-SGD proposed in \cite{Shen2019FasterDD} can decouple communication and computation as well. In \Cref{tab:comparison_iid}, we empirically compare the performance of these Local SGD variants. The results show that given a fixed number of $\cp$, {\alg} always achieves the best test accuracy among all methods, and EAMSGD has significant worse performance than others.  

\begin{table}[t]
    \centering
    \begin{tabular}{c c c c c c}\toprule
    Algorithm & $\cp=1$ & $\cp=2$ & $\cp=8$ & $\cp=24$\\\midrule
    CoCoD-SGD &  $94.98\%$ & $94.99\%$ & $94.05\%$ & $92.54\%$\\
    EAMSGD    &  $94.51\%$ & $93.89\%$ & $92.43\%$ & $89.93\%$ \\
    Ours & $\bm{95.19\%}$ & $\bm{95.16\%}$ & $\bm{94.25\%}$ & $\bm{92.92\%}$ \\\bottomrule 
    \end{tabular}
    \caption{Comparison of Local SGD variants in \textbf{IID} data partition setting. As a reference, fully synchronous SGD achieves a test accuracy of $94.97\%$. The corresponding training loss curves can be found in the longer version.}
    \label{tab:comparison_iid}
\end{table}

\begin{table}[t]
    \centering
    \begin{tabular}{c c c c c c}\toprule
    Algorithm & $\cp=1$ & $\cp=2$ & $\cp=8$ & $\cp=24$\\\midrule
    CoCoD-SGD &  $91.50\%$ & $\bm{91.67\%}$ & Diverges & Diverges \\
    EAMSGD    &  $91.38\%$ & $91.12\%$ & $88.88\%$ & $85.59\%$ \\
    Ours & $\bm{91.56\%}$ & $91.61\%$ & $\bm{91.45\%}$ & $\bm{88.73\%}$ \\\bottomrule 
    \end{tabular}
    \caption{Comparison of Local SGD variants in \textbf{Non-IID} data partition setting. As a reference, fully synchronous SGD achieves a test accuracy of $85.88\%$. The hyper-parameter choices are identical to the IID case.}
    \label{tab:comparison_niid}
\end{table}


\textbf{Non-IID Data Partitions Setting.} We further validate the effectiveness of {\alg} in a non-IID data partitions setting. In particular, each node is assigned with $3125$ training samples, $2000$ of which belong to one class. Thus, the training data on each node is highly skewed. In \Cref{fig:NIID}, observe that both fully synchronous SGD and Local SGD are pretty unstable in this case. {\alg} not only reduces the total training time but also yields better convergence in terms of error-versus-iterations (see \Cref{fig:NIID}(c)). Compared to CoCoD-SGD (see \Cref{tab:comparison_niid}), {\alg} still can achieve comparable test accuracy and overcome the divergence issue when $\cp$ is large.

% \begin{figure}[b]
%     \centering
%     \includegraphics[width=.3\textwidth]{overlap_results.pdf}
%     \caption{Example of the error-runtime trade-off. The proposed algorithm {\alg} significantly improves the Pareto efficiency of communication-efficient SGD. Note that the computation time per epoch is about $0.0$s [TBA]. PowerSGD \cite{vogels2019powersgd} is the state-of-the-art gradient compression technique.}
%     \label{fig:trade-off}
% \end{figure}

==> 4_analysis.tex <==
\section{Convergence Analysis}\label{sec:convergence}
In this section, we will provide a convergence guarantee for {\alg} under non-convex objectives, which are common for deep neural networks. The analysis is based on the following assumptions:
\begin{enumerate}
    \item Each local objective function $\obj_i(\bx):=\Exs_{\bm{s} \sim \mathcal{D}_i}\brackets{\ell(\bx;\bm{s})}$ is L-smooth: $\vecnorm{\tg_i(\bx)-\tg_i(\by)}\leq \lip \vecnorm{\bx - \by}, \forall i\in [1,\nworker]$.
    \item The stochastic gradients are unbiased estimators of local objectives' gradients, \ie, $\Exs_{\xi\sim \mathcal{D}_i}[\sg_i(\bx;\xi)]=\tg_i(\bx)$.
    \item The variance of stochastic gradients is bounded by a non-negative constant: $\Exs_{\xi\sim \mathcal{D}_i}[\vecnorm{\sg_i(\bx;\xi)-\tg_i(\bx)}^2]\leq \vbnd$.
    \item The average deviation of local gradients is bounded by a non-negative constant: $\frac{1}{\nworker}\sum_{i=1}^\nworker \vecnorm{\tg_i(\bx)-\tg(\bx)}^2\leq \kappa^2$.
\end{enumerate}

Formally, we have the following theorem. It can guarantee that {\alg} converges to stationary points of non-convex objective functions.
\begin{thm}\label{thm:main}
Suppose all local models and anchor model are initialized at the same point $\bx_0^{(i)}=\bz_0$ for all $i \in \{1,\dots,\nworker\}$. Under Assumptions 1 to 4, if the learning rate is set as $\lr=\frac{1}{\lip}\sqrt{\frac{\nworker}{K}}$, and the total iterations $K$ satisfies $K \geq 60\nworker\cp^2/\glr^2$, then we have
\begin{align}
    \frac{1}{K}\sum_{k=0}^{K-1}\Exs\brackets{\vecnorm{\tg(\by_k)}^2} 
    \leq& \frac{4\lip[\obj(\by_0)-\obj_\text{inf}]}{(1-\glr)\sqrt{\nworker K}} + \frac{2(1-\glr)\vbnd}{\sqrt{\nworker K}} + \nonumber \\
        & \frac{2\nworker\vbnd}{K}\brackets{\frac{2}{(2-\glr)\glr}\cp-1} + \frac{2\nworker\cp^2\kappa^2}{\glr^2 K} \\
    =& \mathcal{O}\parenth{\frac{1}{\sqrt{\nworker K}}} + \mathcal{O}\parenth{\frac{1}{K}}.
\end{align}
where $\by_k = (1-\glr)\sum_{i=1}^\nworker \bx_k^{(i)} + \glr \bz_k$ and $\obj_\text{inf}$ is the lower bound of the objective value.
\end{thm}
Due to space limitation, please refer to the full version for the proof details. Briefly, the proof technique is inspired by \cite{wang2018cooperative}. The key challenge is that the mixing matrix of {\alg} is column-stochastic instead of doubly- or row-stochastic \cite{Nedic2018network}. It is worth highlighting that the analysis can be generalized to other column stochastic matrices rather than the specific form given in \Cref{eqn:W}. \Cref{thm:main} also shows that when the learning rate is configured properly and the total iterations $K$ is sufficiently large, the error bound of {\alg} will be dominated by $1/\sqrt{\nworker K}$, matching the same rate as fully synchronous SGD.


